Denotational semantics as a foundation for cost recurrence extraction for functional languages

A standard informal method for analyzing the asymptotic complexity of a program is to extract a recurrence that describes its cost in terms of the size of its input, and then to compute a closed-form upper bound on that recurrence. We give a formal account of that method for functional programs in a higher-order language with let-polymorphism. The method consists of two phases. In the first phase, a monadic translation is performed to extract a cost-annotated version of the original program. In the second phase, the extracted program is interpreted in a model. The key feature of this second phase is that different models describe different notions of size. This plays out in several ways. For example, when analyzing functions that take arguments of inductive types, different notions of size may be appropriate depending on the analysis. When analyzing polymorphic functions, our approach shows that one can formally describe the notion of size of an argument in terms of the data that is common to the notions of size for each type instance of the domain type. We give several examples of different models that formally justify various informal cost analyses to show the applicability of our approach.

==> defs.tex <==
%defs.tex

%Lots o' definitions, macros, etc.  This file does *not* include
%LaTeX environments!!  It is usable in either a TeX or a LaTeX file.

%
%MISC. SYMBOLS
%
\def\eqdef{=_{\mathrm{df}}}
\let\intersect=\cap
\let\union=\cup
\let\implies=\rightarrow
\let\Implies=\Rightarrow
\let\iff=\leftrightarrow
\let\Iff=\Leftrightarrow
\let\cross=\times
\def\contradiction{\rightarrow \leftarrow}
\let\isom=\cong
\let\cong=\equiv
\let\ident=\equiv
\let\equiv=\sim
\def\isomto{\mathrel{\hbox{$\to$\kern-.85em\raise1ex\hbox{{$\scriptstyle \isom$}}}}\;}
\def\ndiv{{\not \kern -.05em |\ }}
\let\unique=\downarrow
\let\join\vee
\let\meet\wedge

%
% FUNCTION STUFF
%
\def\comp{\mathbin\circ}
\def\ran{\mathrm{Ran}\;}
\def\dom{\mathrm{Dom}\;}
\def\Ran{\ran}
\def\Dom{\dom}
\def\Ker{\mathrm{Ker}\;}
\def\Im{\mathrm{Im}\;}
\def\id{\mathop{\mathrm{id}}\nolimits}

% MISC MACROS
\def\row#1#2#3{#1_{#2},\ldots,#1_{#3}}
\def\powerset#1{{{\mathcal P}(#1)}}
\def\pwrset{{\mathcal P}}
\def\inv#1{#1^{-1}}

%
% SETS.  Check for AMS fonts.
%
\expandafter\ifx\csname Bbb\endcsname\relax
\def\Reals{\mathbf{R}}
\def\Complexes{\mathbf{C}}
\def\Rationals{\mathbf{Q}}
\def\Integers{\mathbf{Z}}
\else
% \def\Reals{{\Bbb R}}
% \def\Complexes{{\Bbb C}}
% \def\Rationals{{\Bbb Q}}
% \def\Integers{{\Bbb Z}}
\def\Reals{\mathbb{R}}
\def\Complexes{\mathbb{C}}
\def\Rationals{\mathbb{Q}}
\def\Integers{\mathbb{Z}}
\fi
\let\reals=\Reals
\let\complexes=\Complexes
\let\rationals=\Rationals
\let\integers=\Integers

\def\setseparator{\mid}
\newcommand{\seq}[2][\relax]{
  \ifx#1\relax
    \langle#2\rangle
  \else
    \ifx#1\left
      \left\langle#2\right\rangle
    \else
      \csname #1l\endcsname\langle#2\csname #1r\endcsname\rangle
    \fi
  \fi
}
\newcommand{\seqst}[3][\relax]{\seq[#1]{#2\setseparator#3}}
\newcommand{\seqidx}[3][\relax]{\seq[#1]{#2}_{{#3}}}
\newcommand{\set}[2][\relax]{
  \ifx#1\relax
    \{#2\}
  \else
    \ifx#1\left
      \left\{#2\right\}
    \else
      \csname #1l\endcsname\{#2\csname #1r\endcsname\}
    \fi
  \fi
}
\newcommand{\setst}[3][\relax]{\set[#1]{#2\setseparator#3}}
\newcommand{\setidx}[3][\relax]{\set[#1]{#2}_{{#3}}}




==> lambda-defs.tex <==
\def\SL{\mathrm{1}\boldsymbol{\lambda}}
\def\PL{\mathrm{2}\boldsymbol{\lambda}}

\def\App{\mathop{\mathrm{App}}\nolimits}
\let\Ap\App
\def\arrow{\mathbin{\rightarrow}}

\def\be{{\beta\eta}}

\let\ccomp\circ
\def\chord#1{\overline{#1}}
\def\comb#1{\mathsf{#1}}

% \let\den\tmden

\def\eqbeta{=_\beta}
\def\eqbe{=_\be}
\def\eqdef{=_{\mathrm{df}}}

\def\llambda{{\lambda\hskip-.45em\lambda}}	% Semantic lambda

\def\fntype{{\otype\arrow\otype}}
\def\fv{\mathop{\mathrm{fv}}\nolimits}

\def\Id{\mathop{\mathrm{Id}}\nolimits}
\let\ident\cong

\let\ocomp\circ
\def\oftype{\mathbin{:}}
\let\operator\underline
\def\otype{o}

\def\polylc{\boldsymbol{\lambda}\mathbf{2}}

\def\red{\twoheadrightarrow}
\def\redss{\rightarrow}

\def\simplc{\boldsymbol{\lambda}\mathbf{1}}
\def\subst#1#2#3{#1[#2/#3]}
\def\sym#1{\mathsf{#1}}

\def\tmden#1{{\lbrack\!\lbrack{#1}\rbrack\!\rbrack}}
\let\den\tmden
\def\tpden#1{{(\!({#1})\!)}}

\def\uline#1{\underline{#1}}



==> macros.tex <==
\input{defs}

\makeatletter

% \define@key{NDinf}{beta-to}[$\beta_\rightarrow$]{$\beta_\rightarrow$}

\newcommand{\NDinfruledef}[2]{\define@key{NDinf}{#1}[(#2)]{(#2)}}
\newcommand{\NDinfrule}[1]{\setkeys{NDinf}{#1}}

\NDinfruledef{refl}{refl}
\NDinfruledef{trans}{trans}
\NDinfruledef{mon}{mon}
\NDinfruledef{idl}{$+$-idl}
\NDinfruledef{idr}{$+$-idr}
\NDinfruledef{assoc}{$+$-assoc}
\NDinfruledef{beta-to}{$\beta_\rightarrow$}
\NDinfruledef{beta-plus}{$\beta_{\mathord+}$}
\NDinfruledef{beta-times}{$\beta_{\mathord\times}$}
\NDinfruledef{beta-delta}{$\beta_\delta$}
\NDinfruledef{beta-fold}{$\beta_{\delta\cfoldkw}$}
\NDinfruledef{beta-all}{$\beta_\forall$}

\newcommand{\infrulelbl}[1]{%
  % \NDinfruledef{#1}{#2}%
  \hypertarget{#1}{\NDinfrule{#1}}
}
\newcommand{\infruleref}[1]{%
  \hyperlink{#1}{\NDinfrule{#1}}}

\makeatother



\renewcommand{\setst}[3][\relax]{%
  \ifx#1\relax\{\else\csname#1l\endcsname\{\fi%
  #2
  \setseparator
  #3
  \ifx#1\relax\}\else\csname#1r\endcsname\}\fi%
}

\WithSuffix\newcommand\setst*[3][\relax]{%
  \begin{aligned}[t]
  \ifx#1\relax\{\else\csname#1l\endcsname\{\fi%
  &#2 \\
  &\setseparator #3
  \ifx#1\relax\}\else\csname#1r\endcsname\}\fi%
  \end{aligned}
}

\input{lambda-defs}
    \newcommand{\ftv}{\mathrm{ftv}}
    \newcommand{\lsubst}{\{}
    \newcommand{\rsubst}{\}}
	% bind x v = x |-> v
    \newcommand{\bind}[2]{{#1}\mapsto{#2}}
	% \subst e v x = e{x |-> v}
    \renewcommand{\subst}[3]{#1\lsubst\bind{#3}{#2}\rsubst}
	% \esubst e \theta = e{\theta}
    \newcommand{\esubst}[2]{#1\lsubst{#2}\rsubst}
	% \esubst* e \theta = (e){\theta}
    \WithSuffix\newcommand\esubst*[2]{\esubst{(#1)}{#2}}
	% \substfor \sigma x = \sigma/x
	\newcommand{\substfor}[2]{{#1}/{#2}}
	% \tysubst e\theta = e{\theta}
	\newcommand{\tysubst}[2]{{#1}\lsubst{#2}\rsubst}
	% \tysubst* e \sigma \alpha = e{\sigma/\alpha}
	\WithSuffix\newcommand\tysubst*[3]{{#1}\lsubst{\substfor {#2} {#3}}\rsubst}
	% \tysubstsa \delta = \tysubst\delta{\vec\sigma}{\vec\alpha}
	\newcommand{\tysubstsa}[1]{\tysubst*{#1}{\vec\sigma}{\vec\alpha}}

    % Cleaning up notation for closures (source language) and substitution
    % environments (recurrence language).
    \newcommand{\lenv}{\{}
    \newcommand{\renv}{\}}
    \newcommand{\substin}[3]{{#1}{\lenv\substfor{#2}{#3}\renv}}
    \newcommand{\bindto}[2]{{#1}\mapsto{#2}}
    \newcommand{\bindin}[3]{{#1}{\lenv\bindto{#2}{#3}\renv}}
    \newcommand{\extend}[3]{\bindin{#1}{#3}{#2}}
	% \cl e \theta = e\theta
	\newcommand{\cl}[2]{{#1}{#2}}
	% \cl* e \theta = (e)\theta
	\WithSuffix\newcommand\cl*[2]{\cl{(#1)}{#2}}
    % \newcommand{\closurejudge}[3]{{#1}\vdash{#2}\:{#3}\,\skeyw{closure}}
    \newcommand{\closurejudge}[3]{\typejudge{#1}{#2}{{#3}\,\skeyw{closure}}}

    % \sfsubst F \sigma = F[\sigma].
    \newcommand{\sfsubst}[2]{{#1}[{#2}]}

    % \derives E J = E :: J
    \newcommand{\derivation}[1]{\mathcal{#1}}
    \newcommand{\derives}[2]{\mbox{${#1}\mathrel{::}{#2}$}}
    \newcommand{\derE}{\mathcal E}

\newenvironment{proofcases}{%
  \renewcommand{\descriptionlabel}[1]{\hspace\labelsep\underline{\textsc{Case: ##1.}}\enspace}%
  \begin{description}%
}{\end{description}}

\newcommand{\proofcaselabel}[1]%
  {\hspace\labelsep\underline{\textsc{Case: #1.}}\enspace}
\renewenvironment{proofcases}%
    {\begin{list}{}%
      {%
        \renewcommand{\makelabel}{\proofcaselabel}
        \setlength{\labelwidth}{0in}
        \setlength{\leftmargin}{0in}
        \setlength{\itemsep}{2ex}
      }}%
    {\end{list}}

\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\bigmax}{\bigvee}
\newcommand{\bigmeet}{\bigwedge}
\newcommand{\disjunion}{\sqcup}
\newcommand{\smin}[1][{}]{\mathrm{in}^{#1}}
\newcommand{\sminl}{\mathrm{inl}}
\newcommand{\sminr}{\mathrm{inr}}
\newcommand{\bigunion}{\bigcup}
\newcommand{\ordideal}{\mathcal{O}}
\newcommand{\downset}[1][{}]{\mathop{\downarrow^{#1}}\nolimits}
\newcommand{\upset}{\mathop\uparrow}
\newcommand{\bmax}{\vee}
\newcommand{\bmin}{\wedge}
\newcommand{\restr}{\upharpoonright}

\newcommand{\infrule}[1]{(#1)}

%%%
%%% Source language
%%%
\newcommand{\skeyw}[1]{\mathtt{#1}}
\newcommand{\sunit}{\skeyw{unit}}
\newcommand{\stimes}{\times}
\newcommand{\sprod}[2]{{#1}\stimes{#2}}
\newcommand{\ssum}[2]{{#1}+{#2}}
\newcommand{\sarr}[2]{{#1}\to{#2}}
\newcommand{\slfp}[2]{\mu{#1}.#2}
\WithSuffix\newcommand\slfp*[2]{\slfp{#1}{(#2)}}
\newcommand{\sforall}[2]{\forall{#1}.#2}
\newcommand{\ssusp}[1]{{#1}\,\skeyw{susp}}

\newcommand{\sctx}{\Gamma}

\newcommand{\sblank}{\underline{~}}
\newcommand{\striv}{(\,)}
\newcommand{\spair}[2]{(#1, #2)}
\newcommand{\stuple}[1]{(#1)}
\newcommand{\sproj}[2]{\pi_{#1}\,#2}
\WithSuffix\newcommand\sproj*[2]{\pi_{#1}(#2)}
\newcommand{\sinj}[3][{}]{\iota^{#1}_{#2}\,#3}
\WithSuffix\newcommand\sinj*[2]{\sinj{#1}(#2)}
\newcommand{\scasekw}{\skeyw{case}}
\newcommand{\scase}[5]{\skeyw{case}\,#1\,\skeyw{of}\,{#2}.{#3};{#4}.{#5}}
\WithSuffix\newcommand\scase*[3]{\scasekw\,#1\,\skeyw{of}\,\setidx{{#2}.{#3}_i}{i=0,1}}
\newcommand{\sdelaykw}{\skeyw{delay}}
\newcommand{\sforcekw}{\skeyw{force}}
\newcommand{\sdelay}[1]{\sdelaykw\,#1}
\WithSuffix\newcommand\sdelay*[1]{\sdelay{(#1)}}
\newcommand{\sforce}[1]{\sforcekw\,#1}
\WithSuffix\newcommand\sforce*[1]{\sforce{(#1)}}
\newcommand{\slam}[2]{\lambda{#1}.{#2}}
\newcommand{\sapp}[2]{{#1}\,{#2}}
\WithSuffix\newcommand\sapp*[2]{(#1){#2}}
\newcommand{\stylam}[2]{\Lambda{#1}.{#2}}
\newcommand{\styapp}[2]{{#1}\,{#2}}
\newcommand{\sconskw}{\skeyw{c}}
\newcommand{\sdestkw}{\skeyw{d}}
\newcommand{\scons}[2]{\sconskw_{#1}\,{#2}}
\newcommand{\sdest}[2]{\sdestkw_{#1}\,{#2}}
\newcommand{\sletkw}{\skeyw{let}}
\newcommand{\sinkw}{\skeyw{in}}
\newcommand{\slet}[3]{\skeyw{let}\,{#1}={#2}\,\skeyw{in}\,{#3}}
\newcommand\sletmulti[2]{\skeyw{let}\,{#1}\,\skeyw{in}\,{#2}}
\WithSuffix\newcommand\slet*[3]{%
  \begin{aligned}[t]
  &\sletkw\,{#1}={#2} \\
  &\sinkw\,{#3}
  \end{aligned}
}
\newcommand{\sletreckw}{\skeyw{letrec}}
\newcommand{\sletrec}[3]{\sletreckw\,{#1}={#2}\,\sinkw\,{#3}}
\newcommand{\sreckw}{\skeyw{rec}}
\newcommand{\srec}[4]{\sreckw_{#1}\,#2\,\skeyw{of}\,{#3}.{#4}}
\newcommand{\sfoldkw}{\skeyw{fold}}
\newcommand{\sfold}[4]{\sfoldkw_{#1}\,#2\,\skeyw{of}\,{#3}.{#4}}
\newcommand{\smapkw}{\skeyw{map}}
\newcommand{\smap}[4]{\smapkw_{#1}\,{#2}.{#3}\,\skeyw{into}\,{#4}}
\newcommand{\smapvkw}{\skeyw{mapv}}
\newcommand{\smapv}[4]{\smapvkw_{#1}\,{#2}.{#3}\,\skeyw{into}\,{#4}}
\newcommand{\slammap}[5]{\lambda^{\smap{#1}{#2}{#3}\cdot}{#4}.{#5}}
\newcommand{\stickkw}{\skeyw{tick}}

% Standard source-language types.

\newcommand{\sint}{\skeyw{int}}
\newcommand{\snn}[1]{\underline{{#1}}}

\newcommand{\sbool}{\skeyw{bool}}
\newcommand{\strue}{\skeyw{true}}
\newcommand{\sfalse}{\skeyw{false}}
\newcommand{\sif}[3]{\skeyw{if}\,#1\,\skeyw{then}\,#2\,\skeyw{else}\,#3}
\WithSuffix\newcommand\sif*[3]{%
  \begin{aligned}[t]
  &\skeyw{if}\,#1\,\skeyw{then}\,#2 \\
  &\skeyw{else}\,#3
  \end{aligned}
}

\newcommand{\sorder}{\skeyw{order}}
\newcommand{\scaseorder}[4]{%
  \scasekw\,#1\,\skeyw{of}\,\skeyw{LT}.{#2}; 
                                  \skeyw{EQ}.{#3}; 
                                  \skeyw{GT}.{#4}
}
\WithSuffix\newcommand\scaseorder*[4]{%
  \begin{aligned}[t]
  \scasekw\,#1\,\skeyw{of}\,&\skeyw{LT}.{#2}; \\
                            &\skeyw{EQ}.{#3}; \\
                            &\skeyw{GT}.{#4}
  \end{aligned}
}

\newcommand{\snat}{\skeyw{nat}}
\newcommand{\snzero}{\skeyw{Z}}
\newcommand{\snsucc}{\skeyw{S}}
\newcommand{\splus}{\skeyw{plus}}
\newcommand{\snnum}[1]{\skeyw{#1}}

\newcommand{\slist}[1]{{#1}\,\skeyw{list}}
\newcommand{\snlist}{\skeyw{nlist}}
\newcommand{\slnil}{\skeyw{nil}}
\newcommand{\slcons}{\skeyw{cons}}
\newcommand{\slapp}{\skeyw{app}}
\newcommand{\slmap}{\skeyw{map}}
\newcommand{\sltail}{\skeyw{tail}}
\newcommand{\slrev}{\skeyw{rev}}

\newcommand{\stree}[1]{{#1}\,\skeyw{tree}}
\newcommand{\sitree}{\skeyw{itree}}
\newcommand{\snattree}{\stree\snat}
\newcommand{\stemp}{\skeyw{emp}}
\newcommand{\stnode}{\skeyw{node}}

\newcommand{\scopy}{\skeyw{copy}}
\newcommand{\sbstmem}{\skeyw{mem}}
\newcommand{\ssumtree}{\skeyw{sumtree}}

% Pattern-matching
\newcommand{\pmclause}[2]{{#1}\Rightarrow{#2}}
\newcommand{\sfoldpm}[3]{\sfoldkw_{#1}\,#2\,\skeyw{of}\,#3}
\newcommand{\sfoldnat}[3]{\sfoldpm{\snat}{#1}%
  {
    \pmclause{\snzero}{#2} \mid
	\pmclause{\snsucc}{#3}
  }}
\WithSuffix\newcommand\sfoldnat*[3]{\sfoldpm{\snat}{#1}%
  {\begin{aligned}[t]
    & \phantom{{}\mid{}} \pmclause{\snzero}{#2} \\
	& {}\mid \pmclause{\snsucc}{#3}
   \end{aligned}
  }}
\newcommand{\sfoldlist}[4]{\sfoldpm{\slist #1}{#2}%
  {
    \pmclause{\slnil}{#3} \mid
	\pmclause{\slcons}{#4}
  }}
\WithSuffix\newcommand\sfoldlist*[4]{\sfoldpm{\slist #1}{#2}%
  {\begin{aligned}[t]
    & \phantom{{}\mid{}} \pmclause{\slnil}{#3} \\
	& {}\mid \pmclause{\slcons}{#4}
   \end{aligned}
  }}
\newcommand{\sfoldtree}[4]{\sfoldpm{\stree #1}{#2}%
  {
    \pmclause{\stemp}{#3} \mid
	\pmclause{\stnode}{#4}
  }}
\WithSuffix\newcommand\sfoldtree*[4]{\sfoldpm{\stree #1}{#2}%
  {\begin{aligned}[t]
    & \phantom{{}\mid{}} \pmclause{\stemp}{#3} \\
	& {}\mid \pmclause{\stnode}{#4}
   \end{aligned}
  }}
  

\newcommand{\Fmum}{F^{\mathrm{pred}}_{\mu-}}
\newcommand{\Fmu}{F^{\mathrm{pred}}_{\mu}}
\newcommand{\ckeyw}[1]{\mathsf{#1}}
\newcommand{\C}{\ckeyw{C}}
\newcommand{\cunit}{\ckeyw{unit}}
\newcommand{\cprod}[2]{{#1}\times{#2}}
\newcommand{\csum}[2]{{#1}+{#2}}
\newcommand{\carr}[2]{{#1}\to{#2}}
\newcommand{\clfp}[2]{\mu{#1}.#2}
\newcommand{\cforall}[2]{\forall{#1}.#2}

\newcommand{\cblank}{\underline{~}}
\newcommand{\ctriv}{(\,)}
\newcommand{\cpair}[2]{(#1, #2)}
\newcommand{\ctuple}[1]{(#1)}
\newcommand{\cproj}[2]{\pi_{#1}\,#2}
\WithSuffix\newcommand\cproj*[2]{\pi_{#1}(#2)}
\newcommand{\cinj}[3][{}]{\iota^{#1}_{#2}\,#3}
\WithSuffix\newcommand\cinj*[2]{\cinj{#1}(#2)}
\newcommand{\ccasekw}{\ckeyw{case}}
\newcommand{\ccase}[5]{\ckeyw{case}\,#1\,\ckeyw{of}\,{#2}.{#3};{#4}.{#5}}
\newcommand{\ccaset}[7]{\ccase{#1}{(#2\oftype#3)}{#4}{(#5\oftype#6)}{#7}}
\WithSuffix\newcommand\ccase*[3]{\ckeyw{case}\,#1\,\ckeyw{of}\,\{{#2}.{#3}\}_{i=0,1}}
\WithSuffix\newcommand\ccaset*[4]{\ccase*{#1}{(#2\oftype #3)}{#4}}
\newcommand{\clam}[2]{\lambda{#1}.{#2}}
\WithSuffix\newcommand\clam*[3]{\clam{(#1\oftype#2)}{#3}}
\newcommand{\capp}[2]{{#1}\,{#2}}
\WithSuffix\newcommand\capp*[2]{(#1){#2}}
\newcommand{\ctylam}[2]{\Lambda{#1}.{#2}}
\newcommand{\ctyapp}[2]{{#1}\,{#2}}
\WithSuffix\newcommand\ctyapp*[2]{\ctyapp{(#1)}{#2}}
\newcommand{\cconskw}{\ckeyw{c}}
\newcommand{\cdestkw}{\ckeyw{d}}
\newcommand{\ccons}[2]{\cconskw_{#1}\,{#2}}
\WithSuffix\newcommand\ccons*[3]{\capp{\ctyapp{\cconskw_{#1}}{#2}}{#3}}
\newcommand{\cdest}[2]{\cdestkw_{#1}\,{#2}}
\WithSuffix\newcommand\cdest*[3]{\capp{\ctyapp{\cdestkw_{#1}}{#2}}{#3}}
\newcommand{\cletkw}{\ckeyw{let}}
\newcommand{\cinkw}{\ckeyw{in}}
\newcommand{\clet}[3]{\ckeyw{let}\,{#1}={#2}\,\ckeyw{in}\,{#3}}
\newcommand\cletmulti[2]{\ckeyw{let}\,{#1}\,\ckeyw{in}\,{#2}}
\WithSuffix\newcommand\clet*[3]{%
  \begin{aligned}[t]
  &\cletkw\,{#1}={#2} \\
  &\cinkw\,{#3}
  \end{aligned}
}
\newcommand{\creckw}{\ckeyw{rec}}
\newcommand{\crec}[4]{\creckw_{#1}\,#2\,\ckeyw{of}\,{#3}.{#4}}
\newcommand{\cfoldkw}{\ckeyw{fold}}
\newcommand{\cfold}[4]{\cfoldkw_{#1}\,#2\,\ckeyw{of}\,{#3}.{#4}}
\newcommand{\cfixkw}{\ckeyw{fix}}
\newcommand{\cfix}[2]{\cfixkw\,{#1}.{#2}}
\newcommand{\cfixn}[3]{\cfixkw_{#1}\,{#2}.{#3}}
\newcommand{\cmap}[5]{\mbox{${#1}[({#3} : {#2}).{#4}, {#5}]$}}
\WithSuffix\newcommand\cmap*[5]{\cmap{({#1})}{#2}{#3}{#4}{#5}}
\newcommand{\cmapkw}{{\ckeyw{map}}}

\newcommand{\cbindkw}{\mathbin{\mathord\gg\mathord=}}
\newcommand{\cbindignorekw}{\mathbin{\mathord\gg}}
\newcommand{\creturnkw}{\ckeyw{return}}


\newcommand{\cbool}{\ckeyw{bool}}
\newcommand{\ctrue}{\ckeyw{true}}
\newcommand{\cfalse}{\ckeyw{false}}
\newcommand{\cif}[3]{\ckeyw{if}\,#1\,\ckeyw{then}\,#2\,\ckeyw{else}\,#3}
\WithSuffix\newcommand\cif*[3]{%
  \begin{aligned}[t]
  &\ckeyw{if}\,#1\,\ckeyw{then}\,#2 \\
  &\ckeyw{else}\,#3
  \end{aligned}
}

\newcommand{\corder}{\ckeyw{order}}
\newcommand{\ccaseorder}[4]{%
  \ccasekw\,#1\,\ckeyw{of}\,\ckeyw{LT}.{#2}; 
                                  \ckeyw{EQ}.{#3}; 
                                  \ckeyw{GT}.{#4}
}
\WithSuffix\newcommand\ccaseorder*[4]{%
  \begin{aligned}[t]
  \ccasekw\,#1\,\ckeyw{of}\,&\ckeyw{LT}.{#2}; \\
                            &\ckeyw{EQ}.{#3}; \\
                            &\ckeyw{GT}.{#4}
  \end{aligned}
}

\newcommand{\cint}{\ckeyw{int}}
\newcommand{\cnat}{\ckeyw{nat}}
\newcommand{\cnzero}{\ckeyw{Z}}
\newcommand{\cnsucc}{\ckeyw{S}}
\newcommand{\cnnum}[1]{\ckeyw{#1}}
\newcommand{\cplus}{\ckeyw{plus}}
\newcommand{\clist}[1]{{#1}\,\ckeyw{list}}
\newcommand{\cnlist}{\ckeyw{nlist}}
\newcommand{\clnil}{\ckeyw{nil}}
\newcommand{\clcons}{\ckeyw{cons}}
\newcommand{\clapp}{\ckeyw{app}}
\newcommand{\clmap}{\ckeyw{map}}
\newcommand{\clrev}{\ckeyw{rev}}
\newcommand{\ctree}[1]{{#1}\,\ckeyw{tree}}
\newcommand{\citree}{\ckeyw{itree}}
\newcommand{\cnattree}{{\ctree\cnat}}
\newcommand{\ctemp}{\ckeyw{emp}}
\newcommand{\ctnode}{\ckeyw{node}}
\newcommand{\ccopy}{\ckeyw{copy}}
\newcommand{\cbstmem}{\ckeyw{mem}}
\newcommand{\csumtree}{\ckeyw{sumtree}}

\newcommand{\cfoldpm}[3]{\cfoldkw_{#1}\,#2\,\ckeyw{of}\,{#3}}

\newcommand{\ccasenat}[2]{%
  \left\{
  \pmclause{\cnzero}{#1} \mid
  \pmclause{\cnsucc}{#2}
  \right\}
}

\WithSuffix\newcommand\ccasenat*[2]{%
  \left\{
  \begin{aligned}
    & \phantom{{}\mid{}} \pmclause{\cnzero}{#1} \\
    & {}\mid \pmclause{\cnsucc}{#2}
  \end{aligned}
  \right\}
}

\newcommand{\cfoldnat}[4]{%
  \cfoldkw_{\cnat}\,{#2}\,\ckeyw{of}\,{\ccasenat{#3}{#4}}
}

\WithSuffix\newcommand\cfoldnat*[4]{%
  \cfoldkw_{\cnat,{#1}}\,{#2}\,\ckeyw{of}\,{\ccasenat*{#3}{#4}}
}

\newcommand{\ccasetree}[2]{%
  \left\{
  \pmclause{\ctemp}{#1} \mid
  \pmclause{\ctnode}{#2}
  \right\}
}
\WithSuffix\newcommand\ccasetree*[2]{%
  \left\{
  \begin{aligned}
    & \phantom{{}\mid{}} \pmclause{\ctemp}{#1} \\
    & {}\mid \pmclause{\ctnode}{#2}
  \end{aligned}
  \right\}
}

\newcommand{\cfoldtree}[5]{%
  \cfoldkw_{\ctree {#1}}\,{#3}\,\ckeyw{of}\,{\ccasetree{#4}{#5}}
}

\WithSuffix\newcommand\cfoldtree*[5]{%
  \cfoldkw_{\ctree {#1}}\,{#3}\,\ckeyw{of}\,{\ccasetree*{#4}{#5}}
}

\newcommand{\ccaselist}[2]{%
  \left\{
  \pmclause{\clnil}{#1} \mid
  \pmclause{\clcons}{#2}
  \right\}
}
\WithSuffix\newcommand\ccaselist*[2]{%
  \left\{
  \begin{aligned}
    & \phantom{{}\mid{}} \pmclause{\clnil}{#1} \\
    & {}\mid \pmclause{\clcons}{#2}
  \end{aligned}
  \right\}
}

\newcommand{\cfoldlist}[5]{%
  \cfoldkw_{\clist {#1}}\,{#3}\,\ckeyw{of}\,{\ccaselist{#4}{#5}}
}

\WithSuffix\newcommand\cfoldlist*[5]{%
  \cfoldkw_{\clist {#1}}\,{#3}\,\ckeyw{of}\,{\ccaselist*{#4}{#5}}
}

\newcommand{\ccost}[1]{{#1}_c}
% \WithSuffix\newcommand\ccost*{\ckeyw{cost}}
\WithSuffix\newcommand\ccost*[1]{\ccost{(#1)}}
\newcommand{\cpot}[1]{{#1}_p}
% \WithSuffix\newcommand\cpot*{\ckeyw{pot}}
\WithSuffix\newcommand\cpot*[1]{\cpot{(#1)}}
\newcommand{\costpluscpy}[2]{{#1} +_c {#2}}

% Complexity and potential translations.
\newcommand{\ctrans}[1]{\|#1\|}
\newcommand{\ptrans}[1]{\langle\!\langle#1\rangle\!\rangle}
\newcommand{\ptrho}{\ptrans\rho}
\newcommand{\ptsigma}{\ptrans\sigma}
\newcommand{\pttau}{\ptrans\tau}

% Bounding and value bounding relations.
\newcommand\boundedby[1][{}]{\preceq_{#1}}
\newcommand\bounded[3][{}]{\mbox{${#2}\boundedby[#1]{#3}$}}
\newcommand\vboundedby[1][{}]{\boundedby[#1]^{\mathrm{val}}}
\newcommand\vbounded[3][{}]{\mbox{${#2}\vboundedby[#1]{#3}$}}

\newcommand{\TyVar}{\mathrm{TyVar}}
\newcommand{\TmVar}{\mathrm{TmVar}}
\newcommand{\Type}{\mathrm{Type}}
\newcommand{\Val}{\mathrm{Val}}
\newcommand{\TyEnv}{\mathrm{TyEnv}}
\newcommand{\tofinite}{\to_{\mathrm{fin}}}

\newcommand{\cctx}{\Gamma}
\newcommand{\tyvar}{\mathrm{tyvar}}
\newcommand{\ccongctx}{\mathcal C}
\newcommand{\elimctx}[1]{\mathcal E[#1]}
\newcommand{\cconghole}{[\,]}
\newcommand{\szleq}{\leq}
\newcommand{\prejudge}[4]{{#1}\proves {#2}\szleq_{#4} {#3}}

% \newcommand{\U}{\mathbf{U}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\U}{{\mathbf{U}}}
\newcommand{\Usm}{\mathbf{U}_{sm}}
\newcommand{\Ulg}{\mathbf{U}_{lg}}
\WithSuffix\newcommand\Usm*{\Usm^*}
\WithSuffix\newcommand\Ulg*{\Ulg^*}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\Ninf}{\N^\infty}

\newcommand{\defleq}{\sqsubseteq}
\newcommand{\defmax}{\sqcup}
\newcommand{\bigdefmax}{\bigsqcup}

\newcommand{\parto}{\rightharpoonup}
\newcommand{\monto}{\to_{\mathrm{mon}}}

\newcommand{\smcross}{\mathrel{\underline{\times}}}
\newcommand{\smplus}{\mathrel{\underline{+}}}
\newcommand{\smto}{\mathrel{\underline{\mathord\to}}}
\newcommand{\smmu}{\mathord{\underline{\smash\mu}}}
\newcommand{\smforall}{\mathord{\underline{\forall}}}

\newcommand{\smkeyw}[1]{\underline{\smash{\mathrm{#1}}}}
\newcommand{\smProj}[1][{}]{\smkeyw{Proj}_{#1}}
\newcommand{\smPair}[1][{}]{\smkeyw{Pair}_{#1}}
\newcommand{\smCase}[1][{}]{\smkeyw{Case}_{#1}}
\newcommand{\smInj}[1][{}]{\smkeyw{Inj}_{#1}}
\newcommand{\smAbs}[1][{}]{\smkeyw{Abs}_{#1}}
\newcommand{\smApp}[1][{}]{\smkeyw{App}_{#1}}
\newcommand{\smCons}[1][{}]{\smkeyw{C}_{#1}}
\newcommand{\smDest}[1][{}]{\smkeyw{D}_{#1}}
\newcommand{\smMap}[1][{}]{\smkeyw{Map}_{#1}}
\newcommand{\smRec}[1][{}]{\smkeyw{Rec}_{#1}}
\newcommand{\smFold}[1][{}]{\smkeyw{Fold}_{#1}}
\newcommand{\smTyAbs}[1][{}]{\smkeyw{TyAbs}_{#1}}
\newcommand{\smTyApp}[1][{}]{\smkeyw{TyApp}_{#1}}

\newcommand{\smcountkw}{\smkeyw{count}}
\newcommand{\smcount}[2]{\smcountkw_{#1}}
\newcommand{\smsizekw}{\smkeyw{size}}
\newcommand{\smsize}[1]{\smsizekw_{#1}}
\newcommand{\smheightkw}{\smkeyw{height}}
\newcommand{\smheight}[1]{\smheightkw_{#1}}
\newcommand{\smAsPair}[1][{}]{\smkeyw{AsPair}_{#1}}
\newcommand{\smAsInj}[1][{}]{\smkeyw{AsInj}_{#1}}
\newcommand{\smAsFn}[1][{}]{\smkeyw{AsFn}_{#1}}

\newcommand{\smabs}{\mathrm{abs}}
\newcommand{\smconc}{\mathrm{conc}}

\newcommand{\dictionary}[1]{\left\{\begin{aligned}#1\end{aligned}\right\}}

% Relational models.

\newcommand{\relU}{\undertilde{\U}}
\newcommand{\relUsm}{\relU_{sm}}
\newcommand{\relUlg}{\relU_{lg}}
\newcommand{\relD}{\undertilde{D}}

\newcommand{\relcross}{\mathrel{\undertilde{\times}}}
\newcommand{\relplus}{\mathrel{\undertilde{+}}}
\newcommand{\relto}{\mathrel{\undertilde{\to}}}
\newcommand{\relmu}{\mathord{\undertilde{\smash\mu}}}
\newcommand{\relforall}{\mathord{\undertilde{\forall}}}

\newcommand{\relkeyw}[1]{\undertilde{\smash{\mathrm{#1}}}}
\newcommand{\relProj}[1][{}]{\relkeyw{Proj}_{#1}}
\newcommand{\relPair}[1][{}]{\relkeyw{Pair}_{#1}}
\newcommand{\relCase}[1][{}]{\relkeyw{Case}_{#1}}
\newcommand{\relInj}[1][{}]{\relkeyw{Inj}_{#1}}
\newcommand{\relAbs}[1][{}]{\relkeyw{Abs}_{#1}}
\newcommand{\relApp}[1][{}]{\relkeyw{App}_{#1}}
\newcommand{\relCons}[1][{}]{\relkeyw{C}_{#1}}
\newcommand{\relDest}[1][{}]{\relkeyw{D}_{#1}}
\newcommand{\relFold}[1][{}]{\relkeyw{Fold}_{#1}}
\newcommand{\relTyAbs}[1][{}]{\relkeyw{TyAbs}_{#1}}
\newcommand{\relTyApp}[1][{}]{\relkeyw{TyApp}_{#1}}

\WithSuffix\newcommand\mathrel*[1]{\mathrel{(#1)}}

\newcommand{\reln}[2]{{#1}\leftrightarrow{#2}}

% \newcommand{\bind}[2]{{#1}/{#2}}
% \renewcommand{\subst}[3]{{#1}\{{#2}/{#3}\}}
% \newcommand{\extend}[3]{{#1}\{{#2}/{#3}\}}
\newcommand{\env}[1]{\{#1\}}
\WithSuffix\newcommand\env*[2]{\env{\bind{#1}{#2}}}

% \def\den#1#2{\llbracket{#1}\rrbracket{#2}}
\renewcommand\den[3][{}]{{#1}\llbracket{#2}\rrbracket{#3}}

\renewcommand\dom{\mathop{\mathrm{dom}}\nolimits}

% ND comments.
\usepackage{framed}
\usepackage[normalem]{ulem}
\setlength{\marginparwidth}{1.25in}
\reversemarginpar
\newenvironment{ndBlockComment}{\begin{oframed}\noindent ND:\\}{\end{oframed}}
\newcommand{\ndComment}[2][\relax]{\ifx#1\relax\else\uline{#1}\fi\marginpar{\renewcommand{\baselinestretch}{1.0}\tiny ND\ifx#1\relax\else (#1)\fi: {#2}}}
\newcommand{\ndTypo}[1]{\ndComment[#1]{$\longrightarrow$}}
\newcommand{\ndDel}[1]{\sout{#1}\ndComment{$\longrightarrow$}}
\newenvironment{commentary}[1][\relax]{%
  % \begin{leftbar}%
  \begin{list}{}{%
    \setlength{\labelwidth}{0in}\setlength{\labelsep}{0in}
    \addtolength{\rightmargin}{.25in}\small\itshape\singlespacing}%
  \item[\textit{Commentary\ifx#1\relax\else (#1)\fi:\enspace}]\ignorespaces}
  {%
  \end{list}
  % \end{leftbar}
  }

\newenvironment{itemdisp}{%
  \par\noindent
  \begin{minipage}{\linewidth}
}{
  \end{minipage}
  \vskip\belowdisplayskip
}

\newenvironment{itemeq}{%
  \begin{itemdisp}
  \begin{equation*}
}{%
  \end{equation*}
  \end{itemdisp}
}

